Learning to Switch Among Agents in a Team via 2-Layer Markov Decision Processes

Reinforcement learning agents have been mostly developed and evaluated under the assumption that they will operate in a fully autonomous manner -- they will take all actions. In this work, our goal is to develop algorithms that, by learning to switch control between agents, allow existing reinforcement learning agents to operate under different automation levels. To this end, we first formally define the problem of learning to switch control among agents in a team via a 2-layer Markov decision process. Then, we develop an online learning algorithm that uses upper confidence bounds on the agents' policies and the environment's transition probabilities to find a sequence of switching policies. The total regret of our algorithm with respect to the optimal switching policy is sublinear in the number of learning steps and, whenever multiple teams of agents operate in a similar environment, our algorithm greatly benefits from maintaining shared confidence bounds for the environments' transition probabilities and it enjoys a better regret bound than problem-agnostic algorithms. Simulation experiments in an obstacle avoidance task illustrate our theoretical findings and demonstrate that, by exploiting the specific structure of the problem, our proposed algorithm is superior to problem-agnostic algorithms.

==> 061_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  
%For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} %\answerTODO{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusions}.} %\answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work contributes to an extensive body of work on human-machine collaboration. In particular, our results contribute towards establishing the theoretical foundations of switching between agents under uncertainty. While we do not claim that our results will have an immediate practical  impact, we do believe  that semi-autonomous deployment of agents may enhance the operation of cyberphysical systems and have a positive societal impact.} %\answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{} %\answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} %\answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs can be found in appendices.} %\answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have included the code in the supplemental material; also, see Footnote~\ref{footnote.code}.} %\answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We provide details of the experimental setup in Section~\ref{sec:experiments}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We did not report error bars as it would be computationally too expensive to re-run the experiments multiple times.} %\answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Footnote~\ref{footnote.compute}.} %\answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?\answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> 065impact.tex <==
% !TEX root =  human-machine-mdp.tex
A number of technical, societal, and legal challenges have precluded the possibility of using fully autonomous 
reinforcement learning agents in cyberphysical systems. 
%
In our work, we argue that it may be possible to overcome these challenges if reinforcement learning algorithms 
are deployed under lower automation levels and we show that this semi-autonomous deployment may enhance 
the operation of cyberphysical systems. 
%
More broadly, our results suggest that, in sequential decision making, a teams of human and machine agents 
working together working together may achieve better performance than the performance they would achieve 
on their own.

==> ModifiedUCRL2.tex <==
\subsection{UCRL2}
\begin{algorithm}[H]
\small
\caption{Modified UCRL2 algorithm for a finite horizon MDP $\Mcal= (\Scal, \Acal, P, C, L)$.}
\label{alg:ucrl2}
  \begin{algorithmic}[1]
    \REQUIRE Cost $C = [c(s, a)]$, confidence parameter $\delta \in (0, 1)$.
        
    \STATE $(\{N_k(s, a)\}, \{N_k(s, a, s')\}) \gets \textsc{InitializeCounts}{()}$ 
      
     \FOR{$k = 1, \ldots, K$}
     	\FOR{$ s, s' \in \Scal, a \in \Acal$}
     		\STATE \mbox{\bf if} $N_k(s, a) \neq 0$ \mbox{\bf then} $\hat{p}_{k}(s'|s, a) \gets \frac{N_k(s, a, s')}{N_k(s, a)}$	     	\mbox{\bf else} $\hat{p}_{k}(s'|s, a) \gets \frac{1}{|\Scal|}$

			\STATE $\beta_k(s, a, \delta) \gets \sqrt{\frac{14|\Scal|\log\left(\frac{2(k - 1)L|\Acal||\Scal|}{\delta}\right)}{\max\{1, N_k(s, a)\}}}$
		\ENDFOR
		\STATE $\pi^k \gets \textsc{ExtendedValueIteration}{(\hat{p}_{k}, \beta_k, C)}$
		\STATE $s_0\gets \textsc{InitialConditions}{()}$
		\FOR {$t=0, \ldots, L-1$}
			\STATE Take action $a_t = \pi^k_t(s_t)$, and observe next state $s_{t+1}$.
			\STATE $N_k(s_t, a_t) \gets N_k(s_t, a_t) + 1$
			\STATE $N_k(s_t, a_t, s_{t + 1}) \gets N_k(s_t, a_t, s_{t + 1}) + 1$
		\ENDFOR
	\ENDFOR
        \STATE \mbox{\bf Return} $\pi^{K}$
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\small
\caption{\textsc{ExtendedValueIteration}}
\label{alg:evi}
  \begin{algorithmic}[1]
    \REQUIRE Empirical transition distribution $\hat{p}(.|s, a)$, cost $c(s, a)$, and confidence interval $\beta(s, a, \delta)$.
    
    \STATE $\pi \gets \textsc{InitializePolicy}()$,\quad $v\gets \textsc{InitializeValueFunction}()$
    \STATE $n \gets |\Scal|$
    
   	\FOR{$t = T-1, \ldots, 0$}
   		\FOR{$s \in \Scal$}
   			\FOR{$a \in \Acal$}
   				\STATE $s'_1, \ldots, s'_{n} \gets \textsc{Sort}(v_{t+1})$ \hfill \# $v_{t + 1}(s'_1) \leq \ldots \leq v_{t + 1}(s'_n)$
   				
   				\STATE $p(s'_1) \gets \min\{1, \hat{p}(s'_1|s, a) + \frac{\beta(s, a, \delta)}{2}\}$
   				
   				\STATE $p(s'_i) \gets \hat{p}(s'_i|s, a)\; \forall\, 1 < i \leq n$
   				\STATE $l \gets n$
   				\WHILE{$\sum_{s'_i \in \Scal} p(s'_i) > 1$}
   				\STATE $p(s'_l) = \max\{0, 1 - \sum_{s'_i\neq s'_l} p(s'_i)\}$
   				\STATE $l \gets l - 1$
   				\ENDWHILE
		   		\STATE $q(s, a) = c(s, a) + \EE_{s' \sim p}\left[v_{t+1}(s')\right]$
		   	\ENDFOR
		   	\STATE $v_t(s) \gets \min_{a \in \Acal}\{q(s, a)\}$
			\STATE $\pi_t(s) \gets \arg\min_{a \in \Acal}\{q(s, a)\}$
   		\ENDFOR
   	\ENDFOR
   	\STATE \mbox{\bf Return} $\pi$
  \end{algorithmic}
\end{algorithm}


==> RegretProof_main.tex <==
In this proof, we assume that $c_e(s,a)+c_c(d)+c_x(d,d') < 1$ for all $s\in \Scal, a\in \Acal$ and $d,d' \in \Dcal$.
Throughout the proof, we will omit the subscripts $P_{\Dcal}^*, P^*$ in $V_{t\given P_{\Dcal}^*, P^*}$ and write $V_{t}$ instead in case of true agent policies $P_{\Dcal}^*$ and true transition probabilities $ P^*$.
%
%
Then, we define the following quantities:
\begin{align}
      P^k_{\Dcal}& = \argmin_{P_{\Dcal} \in \Pcal^k_\Dcal(\delta)} \min_{P \in \Pcal^k(\delta)} V^{\pi^k}_{1|P_{\Dcal}, P}(s_1, d_0), \label{eq:help-optimal-dynamics1} \\
     P^k & = \argmin_{P \in \Pcal^k(\delta)} V^{\pi^k}_{1|P^k_{\Dcal}, P}(s_1, d_0), \label{eq:help-optimal-dynamics2}\\
      \Delta_k & = V_1^{\pi^k}(s_1, d_0) - V_1^{\pi^*}(s_1, d_0), \label{eq:Delta-def} 
%       t_k & = (k-1)L,\label{eq:tkdef} 
\end{align}
where, recall from Eq.~\ref{eq:learning-to-switch-unknown} that, 
\begin{align*}
\pi^k =\argmin_{\pi} \min_{P_{\Dcal} \in \Pcal^k _{\Dcal}}, \min_{P\in\Pcal^k} V^\pi _{1| P_{\Dcal,P}} (s_1,d_0)
\end{align*}
and, $\Delta_k$ indicates the regret for episode $k$. Hence, we have
\begin{equation*}
    R(T) = \sum_{k=1}^K \Delta_k = \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \in \Pcal_{\Dcal}^k \land P^* \in \Pcal^k) +  \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k)
\end{equation*}
Next, we split the analysis into two parts. We first bound  $\sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \in \Pcal_{\Dcal}^k \land P^* \in \Pcal^k)$ and then bound $ \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k)$.

\noindent --- \emph{Computing the bound on $\sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \in \Pcal_{\Dcal}^k \land P^* \in \Pcal^k)$}

First, we note that 
\begin{align*}
    \Delta_k = V^{\pi^k}_1(s_1, d_0) - V^{\pi^*}_1(s_1, d_0) \leq V^{\pi^k}_1(s_1, d_0) - V_{1|P^k_{\Dcal}, P^k}^{\pi^k}(s_1, d_0)
\end{align*}
This is because 
\begin{equation*}
    V_{1|P^k_{\Dcal}, P^k}^{\pi^k}(s_1, d_0) \ost{(i)}{=} \min_{\pi} \min_{P_{\Dcal} \in \Pcal^k _{\Dcal}} \min_{P \in \Pcal^k  } V^\pi_{1|P_{\Dcal}, P}(s_{1}, d_0) \ost{(ii)}{\leq} \min_{\pi} V^\pi_{1|P^*_{\Dcal}, P^*}(s_{1}, d_0) = V^{\pi^*}_1(s_{1}, d_0),
\end{equation*}
where (i) follows from Eqs.~\ref{eq:help-optimal-dynamics1},~\ref{eq:help-optimal-dynamics2}, and (ii) holds because of the fact that the true transition probabilities $P^*_{\Dcal} \in \Pcal^k_{\Dcal}$ and $P^* \in \Pcal^k$.
%
Next, we use Lemma~\ref{lemma:upper-exp} (Appendix~\ref{app:useful-lemmas}) to bound $\sum_{k=1}^K (V^{\pi^k}_1 (s_1, d_0)- V_{1|P^k_{\Dcal}, P^k}^{\pi^k}(s_{1}, d_0))$.
\begin{equation*}
\sum_{k=1}^K (V^{\pi^k}_1 (s_1,d_0) - V_{1|P^k_{\Dcal}, P^k}^{\pi^k}(s_1, d_0))\leq \sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k_{\Dcal}(s_t, d_t, \delta)\} + \sum_{t=1}^L\min\{1, \beta^k(s_t, a_t \delta)\}\bigg|s_1, d_0\right]
\end{equation*}
Since by assumption,  $c_e(s,a)+c_c(d)+c_x(d,d') < 1$ for all $s\in \Scal, a\in \Acal$ and $d,d' \in \Dcal$,
the worst-case regret is bounded by $T$. Therefore, we have that:
\begin{align}
        \sum_{k=1}^K & \Delta_k\II(P^*_{\Dcal} \in \Pcal_{\Dcal}^k \land P^* \in \Pcal^k)\nn\\
        &\leq \min\left\{T, \sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k_{\Dcal}(s_t, d_t, \delta)\}|s_1 , d_0\right]\right.\nn\\
        &\left.\qquad \qquad + \sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k(s_t, a_t, \delta)\}|s_1, d_0\right] \right\} \nn\\
        & \le \min\left\{T, \sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k_{\Dcal}(s_t, d_t, \delta)\}|s_1 , d_0\right]\right\}\nn\\
        &\qquad  + \min\left\{T,\sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k(s_t, a_t, \delta)\}|s_1, d_0\right] \right\},          
        \label{ineq:split-reg}
\end{align}
%
where, the last inequality follows from Lemma~\ref{lem:minlemma}.
% Now, we aim to bound the first term in the RHS of the above inequality.
Now, we apply Lemma~\ref{lemma:cntbound} to the first term in the RHS of the above inequality:
\begin{equation}
    \sum_{k=1}^K L  \EE\left[\sum_{t=1}^L\min\{1, \beta^k_{\Dcal}(s_t, d_t, \delta)\}\big|s_1, d_0\right]
%     &\ost{(i)}{=} L\sum_{k=1}^K \EE\left[\sum_{t=1}^L\min\left\{1, \sqrt{\frac{2 \log\left(\frac{((k-1)L)^7|\Scal||\Dcal|2^{|\Acal|+1}}{\delta}\right)}{\max\{1, N_k(s_t, d_t)\}}}\right\}\bigg|s_1, d_0\right]\nn\\
%     %
%     &\ost{(ii)}{\leq} L\sum_{k=1}^K \EE\left[\sum_{t=1}^L\min\left\{1, \sqrt{\frac{2 \log\left(\frac{(KL)^7|\Scal||\Dcal|2^{|\Acal|+1}}{\delta}\right)}{\max\{1, N_k(s_t, d_t)\}}}\right\}\right]\nn\\
%     %
% %     &\ost{(iii)}{=} L\sum_{k=1}^K \EE\left[\sum_{t=1}^L\min\{1, \frac{c}{\sqrt{\max\{1, N_k(w_{k, t})\}}}\}\right]\nn\\
%     %
%     & \ost{(iii)}{\leq} 2\sqrt{2}L\sqrt{2 \log\left(\frac{(KL)^7|\Scal||\Dcal|2^{|\Acal|+1}}{\delta}\right)|\Scal||\Dcal|KL}\nn\\
%     &\quad + 2L^2|\Scal||\Dcal|\\
%     & \leq 2\sqrt{2} \sqrt{14|\Acal| \log\left(\frac{(KL)|\Scal||\Dcal|}{\delta}\right)|\Scal||\Dcal|KL}  + 2L^2|\Scal||\Dcal|\nn\\
    \leq \sqrt{112} \sqrt{|\Acal| \log\left(\frac{(KL)|\Scal||\Dcal|}{\delta}\right)|\Scal||\Dcal|KL}  + 2L^2|\Scal||\Dcal| \label{ineq:help}
\end{equation}
which is smaller than
\begin{align} 
12  L \sqrt{|\Scal||\Acal||\Dcal| T\log\left(\frac{|\Scal||\Dcal|T}{\delta}\right)} \label{eq:firstineq}
\end{align}
% % where (i) follows by replacing $\beta_{\Dcal}^k(s_t, d_t, \delta)$ with its definition, (ii) follows by the fact that $(k-1)L \leq KL$, (iii) follows from Lemma~\ref{lemma:cntbound}, in which, we put  $\Wcal := \Scal \times \Dcal$,
% %     $c := \sqrt{2 \log\left(\frac{(KL)^7|\Scal||\Dcal|2^{|\Acal|+1}}{\delta}\right)}$,
% %     $\Tau_k = (w_{k, 1}, \dots, w_{k, L}) := ((s_1, d_1), \dots, (s_L, d_L))$.  
% and (iv) follows by using Lemma~\ref{lemma:cntbound} given the above definitions.
% Further,
% \begin{align}
%     \sqrt{2 \log\left(\frac{(KL)^7|\Scal||\Dcal|2^{|\Acal|+1}}{\delta}\right)|\Scal||\Dcal|KL} &\leq \sqrt{14 \log\left(\frac{(KL)|\Scal||\Dcal|2^{|\Acal| + 1}}{\delta}\right)|\Scal||\Dcal|KL}\nn\\
%     &\leq \sqrt{14|\Acal| \log\left(\frac{(KL)|\Scal||\Dcal|}{\delta}\right)|\Scal||\Dcal|KL} \label{ineq:help2}
% \end{align}
% Then, we plug Eq.~\ref{ineq:help2} in Eq.~\ref{ineq:help}:
% % % Now, due to Eq.~\ref{ineq:help}, we have the following.
% % % \begin{align}
% % % \min&\left\{T,\sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k_{\Dcal}(s_t, d_t, \delta)\}|s_1, d_0 \right]\right\}\nn \\
% % % & {\leq} \min\left\{T,\sqrt{112} L \sqrt{|\Acal||\Scal||\Dcal|T\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)} + 2L^2|\Scal||\Dcal|\right\}\label{eq:minhelp}
% % % % &\ost{(ii)}{\leq} 12  L \sqrt{|\Acal||\Scal||\Dcal|KL \log\left(\frac{(KL)|\Scal||\Dcal|}{\delta}\right)},\label{ineq:first}
% % % \end{align}
% % % Now, if $T \leq 2L^2|\Scal||\Acal||\Dcal|\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)$,
% % % \begin{align}
% % % T^2 \leq 2L^2|\Scal||\Acal||\Dcal|T\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right) \implies
% % % T \leq \sqrt{2}L\sqrt{|\Scal||\Acal||\Dcal|T \log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)}\nn
% % % \end{align}
% % % %
% % % and if $T > 2L^2|\Scal||\Acal||\Dcal|\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)$,
% % % \begin{align}
% % % 2L^2|\Scal| < \frac{\sqrt{2L^2|\Scal||\Acal||\Dcal|T\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)}}{|\Acal||\Dcal|\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)} \leq \sqrt{2}L\sqrt{|\Scal||\Acal||\Dcal|T\log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)}.
% % % \end{align}
% % % %
% % % Thus, the minimum in Eq. \ref{eq:minhelp} is less than
% % % %
% % % \begin{align}
% % % (\sqrt{2} + \sqrt{112}) L \sqrt{|\Scal||\Acal||\Dcal|T\log\left(\frac{|\Scal||\Dcal|T}{\delta}\right)} < 12  L \sqrt{|\Scal||\Acal||\Dcal| T\log\left(\frac{|\Scal||\Dcal|T}{\delta}\right)} \label{eq:firstineq}
% % % \end{align}

% where (i) is due to Eq.~\ref{ineq:help} and (ii) is due to Lemma \ad{TBD}.
A similar analysis can be done for the second term of the RHS of Eq.~\ref{ineq:split-reg}, which would show that,
% Defining $\Wcal = \Scal \times \Acal$ and 
% \begin{align}
%     &c := \sqrt{2 \log\left(\frac{(KL)^7|\Scal||\Acal|2^{|\Scal|+1}}{\delta}\right)}\\
%     &\Tau_k = (w_{k, 1}, \dots, w_{k, L}) := ((s_1, a_1), \dots, (s_L, a_L))
% \end{align}
% We can use the same Lemma~\ref{lemma:cntbound}. Thus,

\begin{equation}
%     \sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k(s_t, a_t, \delta)\}|s_1, d_0\right]&\leq
\min\left\{T,\sum_{k=1}^K L \EE\left[\sum_{t=1}^L\min\{1, \beta^k(s_t, a_t, \delta)\}|s_1, d_0\right] \right\} \le    12L |\Scal|\sqrt{|\Acal|T \log\left(\frac{T|\Scal||\Acal|}{\delta}\right)} \label{ineq:second}.
\end{equation}
%
Combining Eqs.~\ref{ineq:split-reg},~\ref{eq:firstineq} and~\ref{ineq:second}, we can bound the first term of the total regret as follows:
\begin{equation}
    \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \in \Pcal_{\Dcal}^k \land P^* \in \Pcal^k) \leq 12  L \sqrt{|\Acal||\Scal||\Dcal|T \log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)} + 12L|\Scal|\sqrt{|\Acal| T \log\left(\frac{T|\Scal||\Acal|}{\delta}\right)}
    \label{eq:first-term}
\end{equation}
% where $T = KL$.
% 
\noindent --- \emph{Computing the bound on $\sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k)$}

Here, we use a similar approach to ~\cite{jaksch2010near}. Note that
\begin{equation}
    \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) = \sum_{k=1}^{\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor} \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k)+ \sum_{k=\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor+1}^{K} \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k).
\end{equation}
Now, our goal is to show the second term of the RHS of above equation vanishes with high probability. If we succeed, then it holds that, with high probability, $\sum_{k=1}^K  \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k)$ equals the first term of the RHS and then we will be done because
\begin{align}
    \label{eq:hhh10}
    \sum_{k=1}^{\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor} \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) \leq \sum_{k=1}^{\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor} \Delta_k \stackrel{(i)}{\leq}  \left\lfloor\sqrt{\frac{K}{L}}\right\rfloor L = \sqrt{KL},
\end{align}
where (i) follows from the fact that $\Delta_k \leq L$ since we assumed the cost of each step $c_e(s, a) + c_c(d) + c_x(d, d') \leq 1$ for all $s\in \Scal$, $a \in \Acal$, and $d, d' \in \Dcal$.

To prove that $\sum_{k=\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor+1}^{K} \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) = 0$ with high probability, we proceed as follows. By applying Lemma \ref{lemma:p2lm} to $P^*_{\Dcal}$ and $P^*$, we have

\begin{align}
    \text{Pr}(P^*_{\Dcal} \not \in \Pcal^k_{\Dcal}) \leq \frac{\delta}{2{t_k}^6},\; \text{Pr}(P^* \not \in \Pcal^k) \leq \frac{\delta}{2{t_k}^6}
\end{align}
Thus, 
\begin{align}
\label{ineq:addlemmaout}
\prb(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) \leq \text{Pr}(P^*_{\Dcal} \not \in \Pcal^k_{\Dcal}) + \text{Pr}(P^* \not \in \Pcal^k) \leq \frac{\delta}{{t_k}^6}
\end{align}
where $t_k = (k-1)L$ is the end time of episode $k - 1$. Therefore, it follows that
\begin{align} 
\prb\Bigg(\sum_{k=\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor + 1}^{K} \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) = 0\Bigg) & \ost{(i)}{\geq} 1 - \sum_{k=\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor + 1}^{K}  \prb(P^*_{\Dcal} \not \in \Pcal^k_{\Dcal} \lor P^* \not \in \Pcal^k)\nn \\
&  \ost{(ii)}{\geq} 1 - \sum_{k=\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor + 1}^{K}  \frac{\delta}{t_k^6}\nn\\
&\ost{(iii)}{\geq} 1 - \sum_{t=\sqrt{KL}}^{KL}  \frac{\delta}{{t}^6}  \geq 1 - \int_{\sqrt{KL}}^{KL} \frac{\delta}{{t}^6} \geq 1 - \frac{\delta}{5(KL)^{\frac{5}{4}}}.
\end{align}
%
where (i) follows from a union bound, (ii) follows from Eq.~\ref{ineq:addlemmaout} and (iii) holds using that $t_k = (k-1)L$.
%
Hence, with probability at least  $1 - \frac{\delta}{5(KL)^{\frac{5}{4}}}$ we have that 
%
\begin{align}
\sum_{k=\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor + 1}^{K}  \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) = 0.
\end{align}
If we combine the above equation and Eq.~\ref{eq:hhh10}, we can conclude that, with probability at least $1 - \frac{\delta}{5T^{5/4}}$, we have that 
\begin{align}
    \sum_{k=1}^{\left\lfloor\sqrt{\frac{K}{L}}\right\rfloor} \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) \leq \sqrt{T} \label{eq:second-term}
\end{align}
where $T = KL$.
Next, if we combine Eqs.~\ref{eq:first-term} and \ref{eq:second-term}, we have
\begin{align}
    R(T) &= \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \in \Pcal_{\Dcal}^k \land P^* \in \Pcal^k) +  \sum_{k=1}^K \Delta_k\II(P^*_{\Dcal} \not\in \Pcal_{\Dcal}^k \lor P^* \not\in \Pcal^k) \nn\\
%     &\leq 12  L \sqrt{|\Acal||\Scal||\Dcal|T \log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)}+ 12L|\Scal|\sqrt{|\Acal| T \log\left(\frac{T|\Scal||\Acal|}{\delta}\right)} + \sqrt{T}\nn\\
    & \le 13  L \sqrt{|\Acal||\Scal||\Dcal|T \log\left(\frac{T|\Scal||\Dcal|}{\delta}\right)} + 12L|\Scal|\sqrt{|\Acal| T \log\left(\frac{T|\Scal||\Acal|}{\delta}\right)}
\end{align}
Finally, since $\sum_{T=1}^\infty \frac{\delta}{5T^{5/4}} \leq \delta$, with probability at least $1 - \delta$, the above inequality holds. This concludes the proof.
%
For more detailed proof, please refer to supplementary material.
%
%
%
% \newpage
%%%%
%%

